Supervised Learning and Reinforcement Learning of Feedback Models for Reactive Behaviors: Tactile Feedback Testbed

Robots need to be able to adapt to unexpected changes in the environment such that they can autonomously succeed in their tasks. However, hand-designing feedback models for adaptation is tedious, if at all possible, making data-driven methods a promising alternative. In this paper we introduce a full framework for learning feedback models for reactive motion planning. Our pipeline starts by segmenting demonstrations of a complete task into motion primitives via a semi-automated segmentation algorithm. Then, given additional demonstrations of successful adaptation behaviors, we learn initial feedback models through learning from demonstrations. In the final phase, a sample-efficient reinforcement learning algorithm fine-tunes these feedback models for novel task settings through few real system interactions. We evaluate our approach on a real anthropomorphic robot in learning a tactile feedback task.

==> bibliography.tex <==
\begin{thebibliography}{76}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi

\bibitem[{Abadi et~al.(2015)Abadi, Agarwal, Barham, Brevdo, Chen, Citro,
  Corrado, Davis, Dean, Devin, Ghemawat, Goodfellow, Harp, Irving, Isard, Jia,
  Jozefowicz, Kaiser, Kudlur, Levenberg, Mané, Monga, Moore, Murray, Olah,
  Schuster, Shlens, Steiner, Sutskever, Talwar, Tucker, Vanhoucke, Vasudevan,
  Viégas, Vinyals, Warden, Wattenberg, Wicke, Yu and Zheng}]{TensorFlowBib}
Abadi M, Agarwal A, Barham P, Brevdo E, Chen Z, Citro C, Corrado G, Davis A,
  Dean J, Devin M, Ghemawat S, Goodfellow I, Harp A, Irving G, Isard M, Jia Y,
  Jozefowicz R, Kaiser L, Kudlur M, Levenberg J, Mané D, Monga R, Moore S,
  Murray D, Olah C, Schuster M, Shlens J, Steiner B, Sutskever I, Talwar K,
  Tucker P, Vanhoucke V, Vasudevan V, Viégas F, Vinyals O, Warden P,
  Wattenberg M, Wicke M, Yu Y and Zheng X (2015) Tensorflow: Large-scale
  machine learning on heterogeneous distributed systems.

\bibitem[{Abu-Dakka et~al.(2015)Abu-Dakka, Nemec, J{\o}rgensen, Savarimuthu,
  Kr{\"u}ger and Ude}]{Abu_Dakka2015}
Abu-Dakka FJ, Nemec B, J{\o}rgensen JA, Savarimuthu TR, Kr{\"u}ger N and Ude A
  (2015) Adaptation of manipulation skills in physical contact with the
  environment to reference force profiles.
\newblock \emph{Autonomous Robots} 39(2): 199--217.

\bibitem[{{Aung} et~al.(2010){Aung}, {Sim} and {Ng}}]{Aung_TrajAlign_ICPR10}
{Aung} Z, {Sim} K and {Ng} WS (2010) Traj align: A method for precise matching
  of 3-d trajectories.
\newblock In: \emph{2010 20th International Conference on Pattern Recognition}.
  pp. 3818--3821.
\newblock \doi{10.1109/ICPR.2010.930}.

\bibitem[{Bishop(1991)}]{Bishop_1991_RBFNN}
Bishop C (1991) Improving the generalization properties of radial basis
  function neural networks.
\newblock \emph{Neural Computation} 3(4): 579--588.

\bibitem[{Bristow et~al.(2006)Bristow, Tharayil and Alleyne}]{Bristow_ILC}
Bristow DA, Tharayil M and Alleyne AG (2006) A survey of iterative learning
  control.
\newblock \emph{IEEE Control Systems Magazine} 26(3): 96--114.

\bibitem[{{Byravan} et~al.(2014){Byravan}, {Boots}, {Srinivasa} and
  {Fox}}]{Byravan_TCHOMP}
{Byravan} A, {Boots} B, {Srinivasa} SS and {Fox} D (2014) Space-time functional
  gradient optimization for motion planning.
\newblock In: \emph{2014 IEEE International Conference on Robotics and
  Automation (ICRA)}. pp. 6499--6506.
\newblock \doi{10.1109/ICRA.2014.6907818}.

\bibitem[{Celemin et~al.(2019)Celemin, Maeda, Ruiz-del Solar, Peters and
  Kober}]{Celemin2019IJRR_RL_MP_PolicySearch_CorrectiveAdvice}
Celemin CE, Maeda G, Ruiz-del Solar J, Peters J and Kober J (2019)
  Reinforcement learning of motor skills using policy search and human
  corrective advice.
\newblock \emph{International Journal of Robotics Research} OnlineFirst.
\newblock \doi{10.1177/0278364919871998}.

\bibitem[{{Chebotar} et~al.(2019){Chebotar}, {Handa}, {Makoviychuk}, {Macklin},
  {Issac}, {Ratliff} and {Fox}}]{Chebotar_Sim2Real}
{Chebotar} Y, {Handa} A, {Makoviychuk} V, {Macklin} M, {Issac} J, {Ratliff} N
  and {Fox} D (2019) Closing the sim-to-real loop: Adapting simulation
  randomization with real world experience.
\newblock In: \emph{2019 International Conference on Robotics and Automation
  (ICRA)}. pp. 8973--8979.
\newblock \doi{10.1109/ICRA.2019.8793789}.

\bibitem[{Chebotar et~al.(2017)Chebotar, Kalakrishnan, Yahya, Li, Schaal and
  Levine}]{Chebotar_PIGPS}
Chebotar Y, Kalakrishnan M, Yahya A, Li A, Schaal S and Levine S (2017) Path
  integral guided policy search.
\newblock In: \emph{2017 IEEE International Conference on Robotics and
  Automation (ICRA)}. pp. 3381--3388.

\bibitem[{Chebotar et~al.(2014)Chebotar, Kroemer and
  Peters}]{Chebotar_IROS_2014}
Chebotar Y, Kroemer O and Peters J (2014) Learning robot tactile sensing for
  object manipulation.
\newblock In: \emph{IEEE/RSJ International Conference on Intelligent Robots and
  Systems}. pp. 3368--3375.

\bibitem[{Chen and Medioni(1992)}]{Chen_IVC_1992}
Chen Y and Medioni G (1992) Object modelling by registration of multiple range
  images.
\newblock \emph{Image Vision Comput.} 10(3): 145--155.

\bibitem[{Cheng et~al.(2018)Cheng, Mukadam, Issac, Birchfield, Fox, Boots and
  Ratliff}]{cheng2018rmpflow}
Cheng CA, Mukadam M, Issac J, Birchfield S, Fox D, Boots B and Ratliff N (2018)
  {RMP}flow: A computational graph for automatic motion policy generation.
\newblock In: \emph{The 13th International Workshop on the Algorithmic
  Foundations of Robotics}.
\newblock \urlprefix\url{http://arxiv.org/abs/1811.07049}.

\bibitem[{Coates et~al.(2008)Coates, Abbeel and
  Ng}]{Coates_LearningInvertedHelicopter_ICML08}
Coates A, Abbeel P and Ng AY (2008) Learning for control from multiple
  demonstrations.
\newblock In: \emph{Proceedings of the 25th International Conference on Machine
  Learning}, ICML ’08. New York, NY, USA: Association for Computing
  Machinery.
\newblock ISBN 9781605582054, p. 144–151.
\newblock \doi{10.1145/1390156.1390175}.

\bibitem[{Donlon et~al.(2018)Donlon, Dong, Liu, Li, Adelson and
  Rodriguez}]{donlon2018gelslim}
Donlon E, Dong S, Liu M, Li J, Adelson E and Rodriguez A (2018) Gelslim: A
  high-resolution, compact, robust, and calibrated tactile-sensing finger.

\bibitem[{Eppner et~al.(2016)Eppner, H{\"o}fer, Jonschkowski,
  Mart{\'i}n-Mart{\'i}n, Sieverling, Wall and Brock}]{Eppner_LessonAPC_RSS16}
Eppner C, H{\"o}fer S, Jonschkowski R, Mart{\'i}n-Mart{\'i}n R, Sieverling A,
  Wall V and Brock O (2016) Lessons from the amazon picking challenge: Four
  aspects of building robotic systems.
\newblock In: \emph{Proceedings of Robotics: Science and Systems}. AnnArbor,
  Michigan.
\newblock \doi{10.15607/RSS.2016.XII.036}.

\bibitem[{{Ewerton} et~al.(2015){Ewerton}, {Maeda}, {Peters} and
  {Neumann}}]{Ewerton_ProMP_DiffSpeedsExec}
{Ewerton} M, {Maeda} G, {Peters} J and {Neumann} G (2015) Learning motor skills
  from partially observed movements executed at different speeds.
\newblock In: \emph{2015 IEEE/RSJ International Conference on Intelligent
  Robots and Systems (IROS)}. pp. 456--463.
\newblock \doi{10.1109/IROS.2015.7353412}.

\bibitem[{Fod et~al.(2002)Fod, Matari{\'c} and Jenkins}]{fod2002automated}
Fod A, Matari{\'c} MJ and Jenkins OC (2002) Automated derivation of primitives
  for movement classification.
\newblock \emph{Autonomous robots} 12(1): 39--54.

\bibitem[{Gams et~al.(2015)Gams, Denisa and Ude}]{gams2015learning}
Gams A, Denisa M and Ude A (2015) Learning of parametric coupling terms for
  robot-environment interaction.
\newblock In: \emph{IEEE International Conference on Humanoid Robots}. pp.
  304--309.

\bibitem[{Gams et~al.(2009)Gams, Ijspeert, Schaal and
  Lenar{\v{c}}i{\v{c}}}]{gams2009line}
Gams A, Ijspeert AJ, Schaal S and Lenar{\v{c}}i{\v{c}} J (2009) On-line
  learning and modulation of periodic movements with nonlinear dynamical
  systems.
\newblock \emph{Autonomous robots} 27(1): 3--23.

\bibitem[{Gams et~al.(2014{\natexlab{a}})Gams, Nemec, Ijspeert and
  Ude}]{Gams_TransRob_2014}
Gams A, Nemec B, Ijspeert AJ and Ude A (2014{\natexlab{a}}) Coupling movement
  primitives: Interaction with the environment and bimanual tasks.
\newblock \emph{IEEE Transactions on Robotics} 30(4): 816--830.

\bibitem[{Gams et~al.(2014{\natexlab{b}})Gams, Petric, Nemec and
  Ude}]{gams2014learning}
Gams A, Petric T, Nemec B and Ude A (2014{\natexlab{b}}) Learning and
  adaptation of periodic motion primitives based on force feedback and human
  coaching interaction.
\newblock In: \emph{IEEE-RAS International Conference on Humanoid Robots}. pp.
  166--171.

\bibitem[{{Hazara} and {Kyrki}(2016)}]{Hazara_PI2_DMP_InContactSkills}
{Hazara} M and {Kyrki} V (2016) Reinforcement learning for improving imitated
  in-contact skills.
\newblock In: \emph{2016 IEEE-RAS 16th International Conference on Humanoid
  Robots (Humanoids)}. pp. 194--201.
\newblock \doi{10.1109/HUMANOIDS.2016.7803277}.

\bibitem[{Hoffmann et~al.(2014)Hoffmann, Chen, Earl, Mitchell, Salemi and
  Sinapov}]{hoffmann2014adaptive}
Hoffmann H, Chen Z, Earl D, Mitchell D, Salemi B and Sinapov J (2014) Adaptive
  robotic tool use under variable grasps.
\newblock \emph{Robotics and Autonomous Systems} 62(6): 833--846.

\bibitem[{Hoffmann et~al.(2009)Hoffmann, Pastor, Park and
  Schaal}]{Hoffmann_ICRA_2009}
Hoffmann H, Pastor P, Park DH and Schaal S (2009) Biologically-inspired
  dynamical systems for movement generation: Automatic real-time goal
  adaptation and obstacle avoidance.
\newblock In: \emph{IEEE International Conference on Robotics and Automation}.
  pp. 2587--2592.

\bibitem[{Hogan et~al.(2020)Hogan, Ballester, Dong and
  Rodriguez}]{hogan2020tactiledexterity}
Hogan FR, Ballester J, Dong S and Rodriguez A (2020) Tactile dexterity:
  Manipulation primitives with tactile feedback.

\bibitem[{Ijspeert et~al.(2013)Ijspeert, Nakanishi, Hoffmann, Pastor and
  Schaal}]{Ijspeert_NC_2013}
Ijspeert AJ, Nakanishi J, Hoffmann H, Pastor P and Schaal S (2013) Dynamical
  movement primitives: Learning attractor models for motor behaviors.
\newblock \emph{Neural Computation} 25(2): 328--373.

\bibitem[{{Johannink} et~al.(2019){Johannink}, {Bahl}, {Nair}, {Luo}, {Kumar},
  {Loskyll}, {Ojea}, {Solowjow} and
  {Levine}}]{Johannink_Residual_RL_Robot_Control}
{Johannink} T, {Bahl} S, {Nair} A, {Luo} J, {Kumar} A, {Loskyll} M, {Ojea} JA,
  {Solowjow} E and {Levine} S (2019) Residual reinforcement learning for robot
  control.
\newblock In: \emph{2019 International Conference on Robotics and Automation
  (ICRA)}. pp. 6023--6029.
\newblock \doi{10.1109/ICRA.2019.8794127}.

\bibitem[{{Kalakrishnan} et~al.(2011){Kalakrishnan}, {Righetti}, {Pastor} and
  {Schaal}}]{Kalakrishnan_LearnForceControlPolicies}
{Kalakrishnan} M, {Righetti} L, {Pastor} P and {Schaal} S (2011) Learning force
  control policies for compliant manipulation.
\newblock In: \emph{2011 IEEE/RSJ International Conference on Intelligent
  Robots and Systems}. pp. 4639--4644.
\newblock \doi{10.1109/IROS.2011.6095096}.

\bibitem[{{Kappler} et~al.(2018){Kappler}, {Meier}, {Issac}, {Mainprice},
  {Cifuentes}, {Wüthrich}, {Berenz}, {Schaal}, {Ratliff} and
  {Bohg}}]{Kappler_RTPerceptionReactiveMotion_RSS17}
{Kappler} D, {Meier} F, {Issac} J, {Mainprice} J, {Cifuentes} CG, {Wüthrich}
  M, {Berenz} V, {Schaal} S, {Ratliff} N and {Bohg} J (2018) Real-time
  perception meets reactive motion generation.
\newblock \emph{IEEE Robotics and Automation Letters} 3(3): 1864--1871.
\newblock \doi{10.1109/LRA.2018.2795645}.

\bibitem[{Khansari et~al.(2016)Khansari, Klingbeil and
  Khatib}]{Khansari_IJRR_2016}
Khansari M, Klingbeil E and Khatib O (2016) Adaptive human-inspired compliant
  contact primitives to perform surface–surface contact under uncertainty.
\newblock \emph{The International Journal of Robotics Research} 35(13):
  1651--1675.

\bibitem[{Khansari-Zadeh and Billard(2012)}]{Zadeh_AutonRob_2012}
Khansari-Zadeh SM and Billard A (2012) A dynamical system approach to realtime
  obstacle avoidance.
\newblock \emph{Auton. Robots} 32(4): 433--454.

\bibitem[{Kober et~al.(2008)Kober, Mohler and Peters}]{Kober_IROS_2008}
Kober J, Mohler B and Peters J (2008) Learning perceptual coupling for motor
  primitives.
\newblock In: \emph{IEEE/RSJ International Conference on Intelligent Robots and
  Systems}. pp. 834--839.

\bibitem[{Kober and Peters(2011)}]{Kober_PoWER}
Kober J and Peters J (2011) Policy search for motor primitives in robotics.
\newblock \emph{Machine Learning} 84(1): 171--203.

\bibitem[{Kramberger et~al.(2016)Kramberger, Gams, Nemec and
  Ude}]{Kramberger_Humanoids16_GenOrientationDMP}
Kramberger A, Gams A, Nemec B and Ude A (2016) Generalization of orientational
  motion in unit quaternion space.
\newblock In: \emph{IEEE-RAS International Conference on Humanoid Robots}. pp.
  808--813.

\bibitem[{Levine et~al.(2016)Levine, Finn, Darrell and
  Abbeel}]{levine_e2e_deep_visuomotor_policies}
Levine S, Finn C, Darrell T and Abbeel P (2016) End-to-end training of deep
  visuomotor policies.
\newblock \emph{Journal of Machine Learning Research} 17(39): 1--40.

\bibitem[{Levine and Koltun(2013)}]{levine_gps}
Levine S and Koltun V (2013) Guided policy search.
\newblock In: \emph{Proceedings of the 30th International Conference on
  International Conference on Machine Learning - Volume 28}, ICML'13. JMLR.org,
  pp. III--1--III--9.

\bibitem[{Likar et~al.(2015)Likar, Nemec, Žlajpah, Ando and
  Ude}]{Likar_DMPCouplingTermILC}
Likar N, Nemec B, Žlajpah L, Ando S and Ude A (2015) Adaptation of bimanual
  assembly tasks using iterative learning framework.
\newblock In: \emph{2015 IEEE-RAS 15th International Conference on Humanoid
  Robots (Humanoids)}. pp. 771--776.

\bibitem[{Lillicrap et~al.(2015)Lillicrap, Hunt, Pritzel, Heess, Erez, Tassa,
  Silver and Wierstra}]{Lillicrap_DDPG}
Lillicrap TP, Hunt JJ, Pritzel A, Heess N, Erez T, Tassa Y, Silver D and
  Wierstra D (2015) Continuous control with deep reinforcement learning.
\newblock \emph{arXiv preprint arXiv:1509.02971} .

\bibitem[{Lioutikov et~al.(2015)Lioutikov, Neumann, Maeda and
  Peters}]{lioutikov2015probabilistic}
Lioutikov R, Neumann G, Maeda G and Peters J (2015) Probabilistic segmentation
  applied to an assembly task.
\newblock In: \emph{Humanoid Robots (Humanoids), 2015 IEEE-RAS 15th
  International Conference on}. IEEE, pp. 533--540.

\bibitem[{{Meier} et~al.(2011){Meier}, {Theodorou}, {Stulp} and
  {Schaal}}]{Meier_movement_segmentation_library_IROS11}
{Meier} F, {Theodorou} E, {Stulp} F and {Schaal} S (2011) Movement segmentation
  using a primitive library.
\newblock In: \emph{2011 IEEE/RSJ International Conference on Intelligent
  Robots and Systems}. pp. 3407--3412.
\newblock \doi{10.1109/IROS.2011.6094676}.

\bibitem[{Mnih et~al.(2013)Mnih, Kavukcuoglu, Silver, Graves, Antonoglou,
  Wierstra and Riedmiller}]{Mnih_DQN}
Mnih V, Kavukcuoglu K, Silver D, Graves A, Antonoglou I, Wierstra D and
  Riedmiller MA (2013) Playing atari with deep reinforcement learning.
\newblock \emph{CoRR} abs/1312.5602.

\bibitem[{Molchanov et~al.(2019)Molchanov, Chen, H{\"{o}}nig, Preiss, Ayanian
  and Sukhatme}]{Molchanov_Sim2Real}
Molchanov A, Chen T, H{\"{o}}nig W, Preiss JA, Ayanian N and Sukhatme GS (2019)
  Sim-to-(multi)-real: Transfer of low-level robust control policies to
  multiple quadrotors.
\newblock \emph{CoRR} abs/1903.04628.

\bibitem[{Mukadam et~al.(2018)Mukadam, Dong, Yan, Dellaert and
  Boots}]{Mukadam_GPMP2}
Mukadam M, Dong J, Yan X, Dellaert F and Boots B (2018) Continuous-time
  gaussian process motion planning via probabilistic inference.
\newblock \emph{The International Journal of Robotics Research} 37(11):
  1319--1340.
\newblock \doi{10.1177/0278364918790369}.

\bibitem[{Nemec and Ude(2012)}]{nemec2012action}
Nemec B and Ude A (2012) Action sequencing using dynamic movement primitives.
\newblock \emph{Robotica} 30(05): 837--846.

\bibitem[{Niekum et~al.(2013)Niekum, Chitta, Barto, Marthi and
  Osentoski}]{Niekum_SemanticSegmentation_RSS13}
Niekum S, Chitta S, Barto A, Marthi B and Osentoski S (2013) Incremental
  semantically grounded learning from demonstration.
\newblock In: \emph{Proceedings of Robotics: Science and Systems}. Berlin,
  Germany.
\newblock \doi{10.15607/RSS.2013.IX.048}.

\bibitem[{Niekum et~al.(2015)Niekum, Osentoski, Konidaris, Chitta, Marthi and
  Barto}]{niekum2015learning}
Niekum S, Osentoski S, Konidaris G, Chitta S, Marthi B and Barto AG (2015)
  Learning grounded finite-state representations from unstructured
  demonstrations.
\newblock \emph{The International Journal of Robotics Research} 34(2):
  131--157.

\bibitem[{Pairet et~al.(2019)Pairet, Ard{\'{o}}n, Mistry and
  Petillot}]{Pairet_IROS19}
Pairet {\`{E}}, Ard{\'{o}}n P, Mistry M and Petillot YR (2019) Learning
  generalisable coupling terms for obstacle avoidance via low-dimensional
  geometric descriptors.
\newblock \emph{CoRR} abs/1906.09941.

\bibitem[{Paraschos et~al.(2018)Paraschos, Daniel, Peters and
  Neumann}]{Paraschos_ProMP}
Paraschos A, Daniel C, Peters J and Neumann G (2018) Using probabilistic
  movement primitives in robotics.
\newblock \emph{Autonomous Robots} 42(3): 529--551.

\bibitem[{Park et~al.(2012)Park, Pan and Manocha}]{Park_ITOMP_ICAPS12}
Park C, Pan J and Manocha D (2012) Itomp: Incremental trajectory optimization
  for real-time replanning in dynamic environments.
\newblock In: \emph{Proceedings of the Twenty-Second International Conference
  on International Conference on Automated Planning and Scheduling},
  ICAPS’12. AAAI Press, p. 207–215.

\bibitem[{Park et~al.(2008)Park, Hoffmann, Pastor and
  Schaal}]{Park_Humanoids_2008}
Park DH, Hoffmann H, Pastor P and Schaal S (2008) Movement reproduction and
  obstacle avoidance with dynamic movement primitives and potential fields.
\newblock In: \emph{IEEE International Conference on Humanoid Robots}. pp.
  91--98.

\bibitem[{Pastor et~al.(2009)Pastor, Hoffmann, Asfour and
  Schaal}]{Pastor_ICRA_2009}
Pastor P, Hoffmann H, Asfour T and Schaal S (2009) Learning and generalization
  of motor skills by learning from demonstration.
\newblock In: \emph{IEEE International Conference on Robotics and Automation}.
  pp. 763--768.

\bibitem[{Pastor et~al.(2013)Pastor, Kalakrishnan, Meier, Stulp, Buchli,
  Theodorou and Schaal}]{pastor2013dynamic}
Pastor P, Kalakrishnan M, Meier F, Stulp F, Buchli J, Theodorou E and Schaal S
  (2013) From dynamic movement primitives to associative skill memories.
\newblock \emph{Robotics and Autonomous Systems} 61(4): 351--361.

\bibitem[{Pastor et~al.(2011)Pastor, Righetti, Kalakrishnan and
  Schaal}]{pastor_IROS_2011_ASM}
Pastor P, Righetti L, Kalakrishnan M and Schaal S (2011) Online movement
  adaptation based on previous sensor experiences.
\newblock In: \emph{IEEE/RSJ International Conference on Intelligent Robots and
  Systems}. pp. 365--371.

\bibitem[{{Queiβer} et~al.(2018){Queiβer}, {Hammer}, {Ishihara}, {Asada} and
  {Steil}}]{Queisser_ILC_DMP_ICDL18}
{Queiβer} JF, {Hammer} B, {Ishihara} H, {Asada} M and {Steil} JJ (2018) Skill
  memories for parameterized dynamic action primitives on the pneumatically
  driven humanoid robot child affetto.
\newblock In: \emph{2018 Joint IEEE 8th International Conference on Development
  and Learning and Epigenetic Robotics (ICDL-EpiRob)}. pp. 39--45.

\bibitem[{Rai et~al.(2014)Rai, Meier, Ijspeert and Schaal}]{rai2014learning}
Rai A, Meier F, Ijspeert AJ and Schaal S (2014) Learning coupling terms for
  obstacle avoidance.
\newblock In: \emph{IEEE-RAS International Conference on Humanoid Robots}. pp.
  512--518.

\bibitem[{Rai et~al.(2017)Rai, Sutanto, Schaal and
  Meier}]{icra2017_learning_feedback}
Rai A, Sutanto G, Schaal S and Meier F (2017) Learning feedback terms for
  reactive planning and control.
\newblock In: \emph{2017 IEEE International Conference on Robotics and
  Automation (ICRA)}. pp. 2184--2191.
\newblock \doi{10.1109/ICRA.2017.7989252}.

\bibitem[{{Ratliff} et~al.(2015){Ratliff}, {Toussaint} and
  {Schaal}}]{Ratliff_RieMO_ICRA15}
{Ratliff} N, {Toussaint} M and {Schaal} S (2015) Understanding the geometry of
  workspace obstacles in motion optimization.
\newblock In: \emph{2015 IEEE International Conference on Robotics and
  Automation (ICRA)}. pp. 4202--4209.
\newblock \doi{10.1109/ICRA.2015.7139778}.

\bibitem[{{Ratliff} et~al.(2009){Ratliff}, {Zucker}, {Bagnell} and
  {Srinivasa}}]{Ratliff_CHOMP}
{Ratliff} N, {Zucker} M, {Bagnell} JA and {Srinivasa} S (2009) Chomp: Gradient
  optimization techniques for efficient motion planning.
\newblock In: \emph{2009 IEEE International Conference on Robotics and
  Automation}. pp. 489--494.
\newblock \doi{10.1109/ROBOT.2009.5152817}.

\bibitem[{Ratliff et~al.(2018)Ratliff, Issac, Kappler, Birchfield and
  Fox}]{RatliffRMP}
Ratliff ND, Issac J, Kappler D, Birchfield S and Fox D (2018) Riemannian motion
  policies.
\newblock \emph{CoRR} abs/1801.02854.
\newblock \urlprefix\url{http://arxiv.org/abs/1801.02854}.

\bibitem[{Sakoe and Chiba(1978)}]{Sakoe_ASSP_1978}
Sakoe H and Chiba S (1978) Dynamic programming algorithm optimization for
  spoken word recognition.
\newblock \emph{IEEE Transactions on Acoustics, Speech, and Signal Processing}
  26(1): 43--49.

\bibitem[{Srivastava et~al.(2014)Srivastava, Hinton, Krizhevsky, Sutskever and
  Salakhutdinov}]{Srivastava2014_NN_Dropouts}
Srivastava N, Hinton G, Krizhevsky A, Sutskever I and Salakhutdinov R (2014)
  Dropout: A simple way to prevent neural networks from overfitting.
\newblock \emph{J. Mach. Learn. Res.} 15(1): 1929--1958.

\bibitem[{Stulp and Sigaud(2012)}]{Stulp_PI2CMA}
Stulp F and Sigaud O (2012) Path integral policy improvement with covariance
  matrix adaptation.
\newblock In: \emph{Proceedings of the 29th International Coference on
  International Conference on Machine Learning}, ICML'12. USA: Omnipress, pp.
  1547--1554.

\bibitem[{{Stulp} et~al.(2012){Stulp}, {Theodorou} and
  {Schaal}}]{Stulp_2012_DMP_RL}
{Stulp} F, {Theodorou} EA and {Schaal} S (2012) Reinforcement learning with
  sequences of motion primitives for robust manipulation.
\newblock \emph{IEEE Transactions on Robotics} 28(6): 1360--1370.

\bibitem[{{Sundaralingam} et~al.(2019){Sundaralingam}, {Lambert}, {Handa},
  {Boots}, {Hermans}, {Birchfield}, {Ratliff} and
  {Fox}}]{BalaLearningTactileForceEstimationICRA19}
{Sundaralingam} B, {Lambert} AS, {Handa} A, {Boots} B, {Hermans} T,
  {Birchfield} S, {Ratliff} N and {Fox} D (2019) Robust learning of tactile
  force estimation through robot interaction.
\newblock In: \emph{2019 International Conference on Robotics and Automation
  (ICRA)}. pp. 9035--9042.

\bibitem[{Sung et~al.(2017)Sung, Salisbury and Saxena}]{Sung_ICRA_2017}
Sung J, Salisbury JK and Saxena A (2017) Learning to represent haptic feedback
  for partially-observable tasks.
\newblock In: \emph{IEEE International Conference on Robotics and Automation}.
  pp. 2802--2809.

\bibitem[{{Sutanto} et~al.(2019){Sutanto}, {Ratliff}, {Sundaralingam},
  {Chebotar}, {Su}, {Handa} and {Fox}}]{icra2019_learning_tactile_servoing}
{Sutanto} G, {Ratliff} N, {Sundaralingam} B, {Chebotar} Y, {Su} Z, {Handa} A
  and {Fox} D (2019) Learning latent space dynamics for tactile servoing.
\newblock In: \emph{2019 International Conference on Robotics and Automation
  (ICRA)}. pp. 3622--3628.
\newblock \doi{10.1109/ICRA.2019.8793520}.

\bibitem[{Sutanto et~al.(2018)Sutanto, Su, Schaal and
  Meier}]{icra2018_learn_tactile_feedback}
Sutanto G, Su Z, Schaal S and Meier F (2018) Learning sensor feedback models
  from demonstrations via phase-modulated neural networks.
\newblock In: \emph{2018 IEEE International Conference on Robotics and
  Automation (ICRA)}. pp. 1142--1149.
\newblock \doi{10.1109/ICRA.2018.8460986}.

\bibitem[{Tamar et~al.(2016)Tamar, Levine and Abbeel}]{Tamar_VIN}
Tamar A, Levine S and Abbeel P (2016) Value iteration networks.
\newblock \emph{CoRR} abs/1602.02867.

\bibitem[{Theodorou et~al.(2010{\natexlab{a}})Theodorou, Buchli and
  Schaal}]{Theodorou_2010_PI2generalized}
Theodorou E, Buchli J and Schaal S (2010{\natexlab{a}}) A generalized path
  integral control approach to reinforcement learning.
\newblock \emph{J. Mach. Learn. Res.} 11: 3137--3181.

\bibitem[{Theodorou et~al.(2010{\natexlab{b}})Theodorou, Buchli and
  Schaal}]{Theodorou_PI2}
Theodorou E, Buchli J and Schaal S (2010{\natexlab{b}}) Learning policy
  improvements with path integrals.
\newblock In: Teh YW and Titterington M (eds.) \emph{Proceedings of the
  Thirteenth International Conference on Artificial Intelligence and
  Statistics}, \emph{Proceedings of Machine Learning Research}, volume~9. Chia
  Laguna Resort, Sardinia, Italy: PMLR, pp. 828--835.

\bibitem[{{Tian} et~al.(2019){Tian}, {Ebert}, {Jayaraman}, {Mudigonda}, {Finn},
  {Calandra} and {Levine}}]{TianManipulationByFeelICRA19}
{Tian} S, {Ebert} F, {Jayaraman} D, {Mudigonda} M, {Finn} C, {Calandra} R and
  {Levine} S (2019) Manipulation by feel: Touch-based control with deep
  predictive models.
\newblock In: \emph{2019 International Conference on Robotics and Automation
  (ICRA)}. pp. 818--824.

\bibitem[{Tieleman and Hinton(2012)}]{Tieleman2012}
Tieleman T and Hinton G (2012) {Lecture 6.5---RmsProp: Divide the gradient by a
  running average of its recent magnitude}.
\newblock COURSERA: Neural Networks for Machine Learning.

\bibitem[{Ude et~al.(2014)Ude, Nemec, Petric and
  Morimoto}]{Ude_ICRA14_OrientationDMP}
Ude A, Nemec B, Petric T and Morimoto J (2014) Orientation in cartesian space
  dynamic movement primitives.
\newblock In: \emph{IEEE International Conference on Robotics and Automation}.
  pp. 2997--3004.

\bibitem[{Veiga et~al.(2020)Veiga, Edin and
  Peters}]{VeigaGripStabilizationTactileFeedbackSensors20}
Veiga F, Edin B and Peters J (2020) Grip stabilization through independent
  finger tactile feedback control.
\newblock \emph{Sensors} 20(6).
\newblock \doi{10.3390/s20061748}.
\newblock \urlprefix\url{https://www.mdpi.com/1424-8220/20/6/1748}.

\bibitem[{Wettels et~al.(2008)Wettels, Santos, Johansson and Loeb}]{wettels08}
Wettels N, Santos VJ, Johansson RS and Loeb GE (2008) Biomimetic tactile sensor
  array.
\newblock \emph{Advanced Robotics} 22(8): 829--849.
\newblock \doi{10.1163/156855308X314533}.

\bibitem[{{Zhou} and {De la Torre}(2012)}]{Zhou_GTW_CVPR12}
{Zhou} F and {De la Torre} F (2012) Generalized time warping for multi-modal
  alignment of human motion.
\newblock In: \emph{2012 IEEE Conference on Computer Vision and Pattern
  Recognition}. pp. 1282--1289.
\newblock \doi{10.1109/CVPR.2012.6247812}.

\end{thebibliography}

